Spurious instabilities in multiangle simulations of collective flavor conversion

The dense neutrino flux streaming from a core-collapse supernova can undergo self-induced flavor conversion caused by neutrino-neutrino refraction. Numerical studies of these nonlinear effects are challenging because representing the neutrino radiation field by discrete energy and angle bins can easily lead to unphysical solutions. In particular, if the number of angle bins N_a is too small, flavor conversion begins too deep and produces completely spurious results. At the same time, N_a=1 (single-angle approximation) can be a good proxy for the N_a -> infinity limit. Based on a linearized stability analysis, we explain some of the puzzling effects of discrete angle distributions.

==> PaxHeaders.16901/text.tex <==
30 mtime=1355408893.012435536
30 atime=1355409612.953533088
30 ctime=1355408893.066435784

